Visual-Aware Text-to-Speech

Dynamically synthesizing talking speech that actively responds to a listening head is critical during the face-to-face interaction. For example, the speaker could take advantage of the listener's facial expression to adjust the tones, stressed syllables, or pauses. In this work, we present a new visual-aware text-to-speech (VA-TTS) task to synthesize speech conditioned on both textual inputs and sequential visual feedback (e.g., nod, smile) of the listener in face-to-face communication. Different from traditional text-to-speech, VA-TTS highlights the impact of visual modality. On this newly-minted task, we devise a baseline model to fuse phoneme linguistic information and listener visual signals for speech synthesis. Extensive experiments on multimodal conversation dataset ViCo-X verify our proposal for generating more natural audio with scenario-appropriate rhythm and prosody.

==> includes/10-data.tex <==
\section{Data Description} \label{sec:data_desc}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/dataset_example.pdf}
    \caption{An example result of phoneme-listener alignment on ViCo-X dataset. Both the standard Chinese phonemes and IPA are annotated. We visualize the listener frames \textit{before} each phoneme starts and plot the mel spectrogram in log-scale.}
    \label{fig:phoneme_listener_align}
\end{figure*}

To achieve this goal, we use the ViCo-X~\cite{vicox} dataset. Compare to existing TTS dataset (\eg, ..., \etc), ViCo-X possess a unique visual modality maintains the video frames for both the speaker and listener, which make it possible to modeling the impacts from listener to audio.

The dataset is based on Jing Dong Dialogue Corpus (JDDC)~\cite{chen2019jddc}, the large-scale real scenario Chinese E-commerce conversation corpus, as the transcriptions (Mandarin). There are 10 speakers in the dataset and the audios are recorded by high-fidelity microphones (\SI{48}{\kHz}, \SI{16}{\bit} depth).

% convert the text sequence into phoneme sequence: more cites
In ViCo-X, each recording contains accompanying transcriptions in Chinese characters. To alleviate the mispronunciation problem, we convert the text sequence into phoneme sequence~\cite{chen2022g2pw} with an open-source Mandarin grapheme-to-phoneme converter\footnote{\url{https://github.com/GitYCC/g2pW}}. 
% from fast speech 2
Then, to align listener frames to phoneme level audio inputs, instead of extracting the phoneme duration using a pre-trained auto-regreessive TTS model, we use Montreal forced alignment (MFA)~\cite{mcauliffe2017montreal} tool to extract the phoneme duration. An example result of phoneme-listener alignment is shown in~\cref{fig:phoneme_listener_align}.

